Curriculum Manager for Source Selection in Multi-Source Domain Adaptation

The performance of Multi-Source Unsupervised Domain Adaptation depends significantly on the effectiveness of transfer from labeled source domain samples. In this paper, we proposed an adversarial agent that learns a dynamic curriculum for source samples, called Curriculum Manager for Source Selection (CMSS). The Curriculum Manager, an independent network module, constantly updates the curriculum during training, and iteratively learns which domains or samples are best suited for aligning to the target. The intuition behind this is to force the Curriculum Manager to constantly re-measure the transferability of latent domains over time to adversarially raise the error rate of the domain discriminator. CMSS does not require any knowledge of the domain labels, yet it outperforms other methods on four well-known benchmarks by significant margins. We also provide interpretable results that shed light on the proposed method.

==> theory.tex <==
\subsection{CMSS: Theoretical Insights}

We first state the classic generalization bound for domain adaptation~\cite{NIPS2006_2983, NIPS2007_3212}. Let $\cH$ be a hypothesis space of $VC$-dimension $d$. For a given hypothsis class $\cH$, define the symmetric difference operator as $\cH \Delta \cH = \{ h(\bx) \oplus h'(\bx) | h, h' \in \cH \}$. Let $\cD_{src}$, $\cD_{tgt}$ denote the source and target distributions respectively, and $\hat{\cD}_{src}$, $\hat{\cD}_{tgt}$ denote the empirical distribution induced by sample of size $m$ drawn from $\cD_{src}$, $\cD_{tgt}$ respectively. Let $\epsilon_{s}$ ($\epsilon_{t}$) denote the true risk on source (target) domain, and $\hat{\epsilon}_{s}$ ($\hat{\epsilon}_{t}$) denote the empirical risk on source (target) domain. Then with probability at least $1-\delta$, $\forall h \in \cH$ (Theorem 1 of \cite{NIPS2007_3212}),
\begin{align}\label{eq:bound_orig}
    \epsilon_{t}(h) \leq \hat{\epsilon}_{s}(h) + \frac{1}{2} d_{\cH \Delta \cH}(\hat{\cD}_{src}, \hat{\cD}_{tgt}) + C
\end{align}
where $C$ is a constant 
\begin{align*}
    C = \lambda + O \left( \sqrt{ \frac{d\log(m/d) + \log(1/\delta)}{m} } \right)
\end{align*}
Here, $\lambda$ is the optimal combined risk (source + target risk) that can be achieved by hypothesis in $\cH$. Let 
$\{ \bx^{s}_{i} \}_{i=1}^{m}$, $\{ \bx^{t}_{i} \}_{i=1}^{m}$ be the samples in the empirical distributions $\hat{\cD}_{src}$ and $\hat{\cD}_{tgt}$ respectively. Then, $P(\bx^{s}_{i}) = 1/m$ and $P(\bx^{t}_{i}) = 1/m$. The empirical source risk can be written as $\hat{\epsilon}_{s}(h) = 1/m \sum_{i}\hat{\epsilon}_{\bx^{s}_{i}}(h)$

Now consider a reweighted source distribution $\hat{\cD}_{wsrc}$, with $P(\bx^{s}_{i}) = w_{i}$. For $\hat{\cD}_{wsrc}$ to be a valid pmf. Note that $\hat{\cD}_{src}$ and $\hat{\cD}_{wsrc}$ share the same samples, and only differ in weights. The generalization bound for this reweighted distribution can be written as
\begin{align*}
    \epsilon_{t}(h) \leq \sum_{i} w_{i} \hat{\epsilon}_{\bx^{s}_{i}}(h) + \frac{1}{2} d_{\cH \Delta \cH}(\hat{\cD}_{wsrc}, \hat{\cD}_{tgt}) + C
\end{align*}
Since the bound holds for all weight arrays $\bw = [w^{s}_{1}, w^{s}_{2}\hdots w^{s}_{m}]$ in a simplex, we can minimize over $\bw$ to get a tight bound. 
\begin{align}\label{eq:weighted_bound}
    \epsilon_{t}(h) \leq \min_{\bw \in \Delta^{m}} \sum_{i} w_{i} \hat{\epsilon}_{\bx^{s}_{i}}(h) + \frac{1}{2} d_{\cH \Delta \cH}(\hat{\cD}_{wsrc}, \hat{\cD}_{t}) + C
\end{align}
The first term is the weighted risk, and the second term $d_{\cH \Delta \cH}(\hat{\cD}_{wsrc}, \hat{\cD}_{tgt})$ is the weighted symmetric divergence which can be realized using a weighted adversarial loss.
Note that when $\bw = [1/m, 1/m, \hdots 1/m]$, we get the original bound~\eqref{eq:bound_orig}. Hence, the original bound is in the feasible set of the above optimization.


\subsection{Relaxations}
In practice, deep neural networks are used to optimize the bounds presented above. Since the bound~\eqref{eq:weighted_bound} is minimized over the weight vector $\bw$, one trivial solution is to assign non-zero weights only to a very few source samples. In this case, a neural network can overfit to these source samples, which could result in low training risk and low domain divergence. To avoid this trivial case, we present two relaxations:
\begin{itemize}
    \item We use the unweighted loss for the source risk (first term in the bound~\eqref{eq:weighted_bound}).  
    \item For the divergence term, instead of minimizing $\bw$ over all the samples, we optimize only over mini-batches. Hence, for every mini-batch, there is at least one $w_{i}$ which is non-zero. Additionally, we make weights a function of input i.e., $w_{i} = G_{\rho}(\bx^{s}_{i})$, which is realized using a neural network. This will smooth the predictions of $w_{i}$, and make the weight network produce a soft-selection over source samples based on correlation with the target. 
\end{itemize}
Note that the curriculum manager network $G_{\rho}$ discussed in the previous section satisfy these criteria.

